Growth or Decay -- I: universality of the turbulent dynamo saturation

The turbulent small-scale dynamo (SSD) is likely to be responsible for the magnetisation of the interstellar medium (ISM) that we observe in the Universe today. The SSD efficiently converts kinetic energy $E_{\rm kin}$ into magnetic energy $E_{\rm mag} $, and is often used to explain how an initially weak magnetic field with $E_{\rm mag} \ll E_{\rm kin}$ is amplified, and then maintained at a level $E_{\rm mag} \lesssim E_{\rm kin}$. Usually, this process is studied by initialising a weak seed magnetic field and letting the turbulence grow it to saturation. However, in this Part I of the Growth or Decay series, using three-dimensional, visco-resistive magnetohydrodynamical turbulence simulations up to magnetic Reynolds numbers of 2000, we show that the same final state in the integral quantities, energy spectra, and characteristic scales of the magnetic field can also be achieved if initially $E_{\rm mag} \sim E_{\rm kin}$ or even if initially $E_{\rm mag} \gg E_{\rm kin}$. This suggests that the final saturated state of the turbulent dynamo is set by the turbulence and the material properties of the plasma, independent of the initial structure or amplitude of the magnetic field. We discuss the implications this has for the maintenance of magnetic fields in turbulent plasmas and future studies exploring the dynamo saturation.

==> sim_table_backup.tex <==
\begin{table*}
\caption{Main simulation parameters and derived quantities used throughout this study. We refer to \autoref{app:table_notes} for table notes.}
\centering
\begin{tabular}{l r@{}l r@{}l r@{}l c r@{}l r@{}l r@{}l r@{}l}
\hline
\hline
& \multicolumn{4}{c}{Turbulence} & \multicolumn{3}{c}{Mean $\vecB{B}$-Field} & \multicolumn{6}{c}{Fluctuating $\vecB{B}$-Field} & \multicolumn{2}{c}{Total $\vecB{B}$-Field}\\
\hline
\multicolumn{1}{c}{Simulation ID} & \multicolumn{2}{c}{$\M$} & \multicolumn{2}{c}{$\frac{\ell_{\text{cor}, v}}{\ell_0}$} & \multicolumn{2}{c}{$\Mao$} & \multicolumn{1}{c}{$\frac{B_0}{c_s \rho_0^{1/2}}$} & \multicolumn{2}{c}{$\Exp{\frac{\delta B^2}{c_s^2 \rho_0}}_{\V}$} & \multicolumn{2}{c}{$\Exp{\left(\frac{\dB\cdot\Bo}{c_s^2 \rho_0}\right)^2 }^{1/2}_{\V}$} & \multicolumn{2}{c}{$\Maturb$} & \multicolumn{2}{c}{$\Matot$}\\
\multicolumn{1}{c}{(1)} & \multicolumn{2}{c}{(2)} & \multicolumn{2}{c}{(3)} & \multicolumn{2}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{2}{c}{(6)} & \multicolumn{2}{c}{(7)} & \multicolumn{2}{c}{(8)} & \multicolumn{2}{c}{(9)}\\
\hline
\texttt{M05MA001}&$0.567$ &$_{-0.07}^{+0.02}$&$1.48$ &$_{-0.07}^{+0.05}$&$0.0113$ &$_{-0.001}^{+0.0003}$&$177.0$&$0.000191$ &$_{-0.005}^{+0.004}$&$2.32$ &$_{-0.5}^{+0.4}$&$392.0$ &$_{-40.0}^{+20.0}$&$0.0113$ &$_{-0.001}^{+0.0003}$\\\texttt{M05MA01}&$0.566$ &$_{-0.07}^{+0.02}$&$1.47$ &$_{-0.07}^{+0.05}$&$0.113$ &$_{-0.01}^{+0.004}$&$17.7$&$0.0181$ &$_{-0.04}^{+0.03}$&$2.23$ &$_{-0.4}^{+0.3}$&$35.6$ &$_{-2.0}^{+2.0}$&$0.113$ &$_{-0.01}^{+0.004}$\\\texttt{M05MA05}&$0.534$ &$_{-0.04}^{+0.004}$&$1.44$ &$_{-0.07}^{+0.02}$&$0.534$ &$_{-0.04}^{+0.004}$&$3.54$&$0.233$ &$_{-0.08}^{+0.05}$&$1.16$ &$_{-0.1}^{+0.05}$&$7.28$ &$_{-0.2}^{+0.3}$&$0.544$ &$_{-0.05}^{+0.005}$\\\texttt{M05MA1}&$0.469$ &$_{-0.05}^{+0.01}$&$0.953$ &$_{-0.005}^{+0.02}$&$0.938$ &$_{-0.1}^{+0.03}$&$1.77$&$1.2$ &$_{-0.3}^{+0.1}$&$1.0$ &$_{-0.07}^{+0.08}$&$2.75$ &$_{-0.2}^{+0.1}$&$0.974$ &$_{-0.08}^{+0.07}$\\\texttt{M05MA2}&$0.462$ &$_{-0.03}^{+0.03}$&$0.783$ &$_{-0.03}^{+0.06}$&$1.85$ &$_{-0.1}^{+0.1}$&$0.886$&$3.17$ &$_{-0.3}^{+0.3}$&$0.871$ &$_{-0.07}^{+0.03}$&$1.67$ &$_{-0.08}^{+0.2}$&$1.59$ &$_{-0.09}^{+0.2}$\\\texttt{M05MA4}&$0.473$ &$_{-0.03}^{+0.06}$&$0.838$ &$_{-0.03}^{+0.03}$&$3.79$ &$_{-0.2}^{+0.5}$&$0.443$&$3.12$ &$_{-0.2}^{+0.2}$&$0.415$ &$_{-0.009}^{+0.02}$&$1.98$ &$_{-0.2}^{+0.2}$&$2.1$ &$_{-0.2}^{+0.4}$\\\texttt{M05MA6}&$0.483$ &$_{-0.03}^{+0.06}$&$0.904$ &$_{-0.03}^{+0.03}$&$5.8$ &$_{-0.4}^{+0.8}$&$0.295$&$2.74$ &$_{-0.1}^{+0.09}$&$0.256$ &$_{-0.006}^{+0.01}$&$2.32$ &$_{-0.1}^{+0.4}$&$2.51$ &$_{-0.2}^{+0.5}$\\\texttt{M05MA8}&$0.502$ &$_{-0.02}^{+0.06}$&$0.907$ &$_{-0.02}^{+0.05}$&$8.03$ &$_{-0.3}^{+1.0}$&$0.222$&$2.47$ &$_{-0.2}^{+0.1}$&$0.192$ &$_{-0.01}^{+0.009}$&$2.76$ &$_{-0.1}^{+0.3}$&$2.99$ &$_{-0.2}^{+0.3}$\\\texttt{M05MA10}&$0.514$ &$_{-0.03}^{+0.06}$&$0.934$ &$_{-0.03}^{+0.02}$&$10.3$ &$_{-0.5}^{+1.0}$&$0.177$&$2.24$ &$_{-0.07}^{+0.1}$&$0.145$ &$_{-0.006}^{+0.01}$&$3.05$ &$_{-0.2}^{+0.4}$&$3.18$ &$_{-0.1}^{+0.4}$\\\texttt{M05MA100}&$0.637$ &$_{-0.05}^{+0.09}$&$0.889$ &$_{-0.03}^{+0.04}$&$127.0$ &$_{-10.0}^{+20.0}$&$0.0177$&$0.721$ &$_{-0.3}^{+0.1}$&$0.00852$ &$_{-0.001}^{+0.0008}$&$7.9$ &$_{-1.0}^{+3.0}$&$7.92$ &$_{-1.0}^{+3.0}$\\\texttt{M05MA1000}&$0.672$ &$_{-0.05}^{+0.07}$&$0.835$ &$_{-0.04}^{+0.03}$&$1340.0$ &$_{-100.0}^{+100.0}$&$0.00177$&$0.36$ &$_{-0.3}^{+0.2}$&$0.000613$ &$_{-0.0002}^{+0.0001}$&$11.8$ &$_{-3.0}^{+8.0}$&$11.8$ &$_{-3.0}^{+8.0}$\\\texttt{M2MA001}&$1.9$ &$_{-0.06}^{+0.04}$&$1.34$ &$_{-0.09}^{+0.02}$&$0.0095$ &$_{-0.0003}^{+0.0002}$&$709.0$&$0.000879$ &$_{-0.003}^{+0.02}$&$18.7$ &$_{-2.0}^{+9.0}$&$498.0$ &$_{-30.0}^{+20.0}$&$0.00943$ &$_{-0.0003}^{+0.0002}$\\\texttt{M2MA01}&$1.85$ &$_{-0.02}^{+0.06}$&$1.37$ &$_{-0.1}^{+0.03}$&$0.0926$ &$_{-0.001}^{+0.003}$&$70.9$&$0.0989$ &$_{-0.03}^{+0.1}$&$18.4$ &$_{-1.0}^{+4.0}$&$41.1$ &$_{-3.0}^{+2.0}$&$0.0917$ &$_{-0.001}^{+0.003}$\\\texttt{M2MA05}&$2.24$ &$_{-0.09}^{+0.07}$&$1.26$ &$_{-0.06}^{+0.08}$&$0.561$ &$_{-0.02}^{+0.02}$&$14.2$&$6.81$ &$_{-0.3}^{+0.3}$&$20.6$ &$_{-2.0}^{+3.0}$&$5.28$ &$_{-0.3}^{+0.3}$&$0.575$ &$_{-0.03}^{+0.01}$\\\texttt{M2MA1}&$1.98$ &$_{-0.09}^{+0.1}$&$0.845$ &$_{-0.02}^{+0.02}$&$0.989$ &$_{-0.05}^{+0.05}$&$7.09$&$25.3$ &$_{-1.0}^{+0.3}$&$16.3$ &$_{-1.0}^{+0.7}$&$2.47$ &$_{-0.2}^{+0.2}$&$1.01$ &$_{-0.06}^{+0.05}$\\\texttt{M2MA2}&$1.95$ &$_{-0.2}^{+0.2}$&$0.815$ &$_{-0.04}^{+0.04}$&$1.95$ &$_{-0.2}^{+0.2}$&$3.54$&$40.6$ &$_{-0.9}^{+0.6}$&$12.3$ &$_{-1.0}^{+0.7}$&$1.73$ &$_{-0.07}^{+0.4}$&$1.54$ &$_{-0.1}^{+0.1}$\\\texttt{M2MA4}&$2.07$ &$_{-0.1}^{+0.2}$&$0.92$ &$_{-0.04}^{+0.02}$&$4.13$ &$_{-0.3}^{+0.5}$&$1.77$&$37.0$ &$_{-0.3}^{+0.3}$&$5.88$ &$_{-0.3}^{+0.4}$&$2.39$ &$_{-0.4}^{+0.1}$&$2.39$ &$_{-0.4}^{+0.3}$\\\texttt{M2MA6}&$2.09$ &$_{-0.2}^{+0.2}$&$0.946$ &$_{-0.05}^{+0.02}$&$6.26$ &$_{-0.6}^{+0.6}$&$1.18$&$33.8$ &$_{-0.4}^{+0.5}$&$3.83$ &$_{-0.1}^{+0.1}$&$2.45$ &$_{-0.3}^{+0.5}$&$2.68$ &$_{-0.5}^{+0.6}$\\\texttt{M2MA8}&$2.05$ &$_{-0.2}^{+0.09}$&$0.945$ &$_{-0.02}^{+0.04}$&$8.21$ &$_{-0.7}^{+0.4}$&$0.886$&$21.5$ &$_{-0.3}^{+0.3}$&$2.39$ &$_{-0.1}^{+0.1}$&$3.44$ &$_{-0.3}^{+0.2}$&$3.91$ &$_{-0.3}^{+0.2}$\\\texttt{M2MA10}&$2.11$ &$_{-0.2}^{+0.1}$&$0.987$ &$_{-0.03}^{+0.03}$&$10.5$ &$_{-1.0}^{+0.7}$&$0.709$&$18.4$ &$_{-0.1}^{+0.3}$&$1.74$ &$_{-0.04}^{+0.1}$&$4.07$ &$_{-0.6}^{+0.3}$&$4.65$ &$_{-0.9}^{+0.4}$\\\texttt{M2MA100}&$2.36$ &$_{-0.2}^{+0.1}$&$1.01$ &$_{-0.02}^{+0.03}$&$118.0$ &$_{-8.0}^{+6.0}$&$0.0709$&$3.3$ &$_{-0.5}^{+0.08}$&$0.0729$ &$_{-0.006}^{+0.003}$&$16.1$ &$_{-2.0}^{+3.0}$&$17.0$ &$_{-3.0}^{+4.0}$\\\texttt{M2MA1000}&$2.37$ &$_{-0.1}^{+0.08}$&$0.999$ &$_{-0.05}^{+0.01}$&$1180.0$ &$_{-70.0}^{+40.0}$&$0.00709$&$0.276$ &$_{-0.3}^{+0.3}$&$0.00214$ &$_{-0.0007}^{+0.0005}$&$61.9$ &$_{-20.0}^{+40.0}$&$62.8$ &$_{-20.0}^{+40.0}$\\\texttt{M4MA01}&$4.03$ &$_{-0.5}^{+0.06}$&$1.39$ &$_{-0.09}^{+0.05}$&$0.101$ &$_{-0.01}^{+0.002}$&$142.0$&$0.838$ &$_{-0.4}^{+0.2}$&$106.0$ &$_{-20.0}^{+9.0}$&$36.5$ &$_{-3.0}^{+3.0}$&$0.1$ &$_{-0.01}^{+0.002}$\\\texttt{M4MA05}&$4.08$ &$_{-0.1}^{+0.04}$&$1.27$ &$_{-0.1}^{+0.04}$&$0.51$ &$_{-0.01}^{+0.005}$&$28.4$&$24.4$ &$_{-0.6}^{+0.4}$&$74.1$ &$_{-7.0}^{+7.0}$&$4.94$ &$_{-0.4}^{+0.3}$&$0.513$ &$_{-0.01}^{+0.007}$\\\texttt{M4MA1}&$4.12$ &$_{-0.4}^{+0.5}$&$0.832$ &$_{-0.04}^{+0.04}$&$1.03$ &$_{-0.09}^{+0.1}$&$14.2$&$84.3$ &$_{-2.0}^{+2.0}$&$61.9$ &$_{-10.0}^{+7.0}$&$2.49$ &$_{-0.1}^{+0.3}$&$1.02$ &$_{-0.1}^{+0.05}$\\\texttt{M4MA2}&$4.02$ &$_{-0.3}^{+0.2}$&$0.846$ &$_{-0.02}^{+0.04}$&$2.01$ &$_{-0.1}^{+0.08}$&$7.09$&$125.0$ &$_{-1.0}^{+1.0}$&$43.4$ &$_{-6.0}^{+2.0}$&$1.93$ &$_{-0.1}^{+0.2}$&$1.49$ &$_{-0.1}^{+0.2}$\\\texttt{M4MA4}&$4.03$ &$_{-0.4}^{+0.2}$&$0.916$ &$_{-0.03}^{+0.02}$&$4.03$ &$_{-0.4}^{+0.2}$&$3.54$&$109.0$ &$_{-0.5}^{+0.2}$&$20.3$ &$_{-0.5}^{+2.0}$&$2.38$ &$_{-0.3}^{+0.1}$&$2.41$ &$_{-0.3}^{+0.1}$\\\texttt{M4MA6}&$3.97$ &$_{-0.4}^{+0.2}$&$0.959$ &$_{-0.02}^{+0.02}$&$5.96$ &$_{-0.6}^{+0.3}$&$2.36$&$76.3$ &$_{-0.6}^{+0.3}$&$11.7$ &$_{-0.4}^{+0.7}$&$2.94$ &$_{-0.3}^{+0.4}$&$3.29$ &$_{-0.2}^{+0.4}$\\\texttt{M4MA8}&$4.05$ &$_{-0.5}^{+0.08}$&$0.979$ &$_{-0.03}^{+0.02}$&$8.1$ &$_{-1.0}^{+0.2}$&$1.77$&$68.5$ &$_{-0.4}^{+0.6}$&$8.38$ &$_{-0.3}^{+0.3}$&$3.41$ &$_{-0.6}^{+0.3}$&$4.15$ &$_{-1.0}^{+0.4}$\\\texttt{M4MA10}&$3.91$ &$_{-0.2}^{+0.2}$&$0.994$ &$_{-0.01}^{+0.03}$&$9.78$ &$_{-0.6}^{+0.5}$&$1.42$&$59.7$ &$_{-0.2}^{+0.2}$&$6.27$ &$_{-0.3}^{+0.2}$&$3.69$ &$_{-0.1}^{+0.3}$&$4.23$ &$_{-0.3}^{+0.9}$\\\texttt{M4MA100}&$4.21$ &$_{-0.08}^{+0.2}$&$1.02$ &$_{-0.02}^{+0.03}$&$105.0$ &$_{-2.0}^{+5.0}$&$0.142$&$6.29$ &$_{-0.4}^{+0.4}$&$0.203$ &$_{-0.01}^{+0.01}$&$21.0$ &$_{-2.0}^{+3.0}$&$24.2$ &$_{-2.0}^{+5.0}$\\\texttt{M4MA1000}&$4.31$ &$_{-0.2}^{+0.1}$&$1.05$ &$_{-0.01}^{+0.02}$&$1080.0$ &$_{-50.0}^{+30.0}$&$0.0142$&$0.391$ &$_{-0.3}^{+0.4}$&$0.00519$ &$_{-0.001}^{+0.001}$&$115.0$ &$_{-40.0}^{+20.0}$&$128.0$ &$_{-50.0}^{+30.0}$\\\texttt{M6MA01}&$6.96$ &$_{-0.8}^{+0.5}$&$1.35$ &$_{-0.04}^{+0.05}$&$0.116$ &$_{-0.01}^{+0.008}$&$213.0$&$3.86$ &$_{-0.7}^{+0.3}$&$325.0$ &$_{-60.0}^{+20.0}$&$29.0$ &$_{-3.0}^{+4.0}$&$0.115$ &$_{-0.01}^{+0.008}$\\\texttt{M6MA05}&$6.44$ &$_{-0.1}^{+0.2}$&$1.21$ &$_{-0.04}^{+0.02}$&$0.536$ &$_{-0.01}^{+0.02}$&$42.5$&$58.0$ &$_{-0.7}^{+1.0}$&$169.0$ &$_{-10.0}^{+10.0}$&$5.02$ &$_{-0.3}^{+0.3}$&$0.535$ &$_{-0.01}^{+0.01}$\\\texttt{M6MA1}&$6.01$ &$_{-0.8}^{+0.8}$&$0.844$ &$_{-0.02}^{+0.04}$&$1.0$ &$_{-0.1}^{+0.1}$&$21.3$&$157.0$ &$_{-4.0}^{+1.0}$&$121.0$ &$_{-20.0}^{+10.0}$&$2.73$ &$_{-0.2}^{+0.2}$&$0.937$ &$_{-0.2}^{+0.1}$\\\texttt{M6MA2}&$5.81$ &$_{-0.3}^{+0.3}$&$0.844$ &$_{-0.03}^{+0.03}$&$1.94$ &$_{-0.09}^{+0.1}$&$10.6$&$217.0$ &$_{-0.5}^{+2.0}$&$83.7$ &$_{-5.0}^{+9.0}$&$2.1$ &$_{-0.1}^{+0.2}$&$1.58$ &$_{-0.09}^{+0.09}$\\\texttt{M6MA4}&$6.23$ &$_{-0.4}^{+0.1}$&$0.94$ &$_{-0.01}^{+0.02}$&$4.15$ &$_{-0.3}^{+0.08}$&$5.32$&$202.0$ &$_{-2.0}^{+0.8}$&$42.8$ &$_{-5.0}^{+2.0}$&$2.55$ &$_{-0.2}^{+0.2}$&$2.53$ &$_{-0.2}^{+0.3}$\\\texttt{M6MA6}&$5.96$ &$_{-0.6}^{+0.4}$&$0.946$ &$_{-0.01}^{+0.02}$&$5.96$ &$_{-0.6}^{+0.4}$&$3.54$&$168.0$ &$_{-1.0}^{+1.0}$&$25.8$ &$_{-2.0}^{+3.0}$&$2.82$ &$_{-0.2}^{+0.3}$&$3.04$ &$_{-0.2}^{+0.3}$\\\texttt{M6MA8}&$5.96$ &$_{-0.5}^{+0.2}$&$0.979$ &$_{-0.01}^{+0.01}$&$7.95$ &$_{-0.6}^{+0.2}$&$2.66$&$139.0$ &$_{-0.9}^{+0.3}$&$17.4$ &$_{-0.6}^{+1.0}$&$3.39$ &$_{-0.4}^{+0.2}$&$3.73$ &$_{-0.4}^{+0.2}$\\\texttt{M6MA10}&$5.99$ &$_{-0.5}^{+0.2}$&$0.99$ &$_{-0.02}^{+0.02}$&$9.99$ &$_{-0.8}^{+0.4}$&$2.13$&$124.0$ &$_{-1.0}^{+0.5}$&$12.6$ &$_{-0.4}^{+1.0}$&$3.82$ &$_{-0.6}^{+0.8}$&$4.11$ &$_{-0.7}^{+1.0}$\\\texttt{M8MA01}&$8.7$ &$_{-0.9}^{+0.09}$&$1.49$ &$_{-0.1}^{+0.02}$&$0.109$ &$_{-0.01}^{+0.001}$&$284.0$&$4.53$ &$_{-0.7}^{+0.4}$&$488.0$ &$_{-90.0}^{+40.0}$&$32.0$ &$_{-4.0}^{+4.0}$&$0.108$ &$_{-0.01}^{+0.001}$\\\texttt{M8MA05}&$8.35$ &$_{-0.3}^{+0.2}$&$1.14$ &$_{-0.02}^{+0.02}$&$0.522$ &$_{-0.02}^{+0.01}$&$56.7$&$90.2$ &$_{-0.6}^{+1.0}$&$278.0$ &$_{-30.0}^{+20.0}$&$5.01$ &$_{-0.4}^{+0.3}$&$0.505$ &$_{-0.03}^{+0.01}$\\\texttt{M8MA1}&$8.16$ &$_{-1.0}^{+0.6}$&$0.837$ &$_{-0.03}^{+0.04}$&$1.02$ &$_{-0.1}^{+0.08}$&$28.4$&$257.0$ &$_{-4.0}^{+2.0}$&$205.0$ &$_{-20.0}^{+10.0}$&$2.74$ &$_{-0.3}^{+0.3}$&$0.92$ &$_{-0.1}^{+0.07}$\\\texttt{M8MA2}&$8.15$ &$_{-0.5}^{+0.4}$&$0.863$ &$_{-0.03}^{+0.03}$&$2.04$ &$_{-0.1}^{+0.1}$&$14.2$&$395.0$ &$_{-1.0}^{+1.0}$&$148.0$ &$_{-8.0}^{+7.0}$&$2.25$ &$_{-0.2}^{+0.2}$&$1.59$ &$_{-0.2}^{+0.1}$\\\texttt{M8MA4}&$7.99$ &$_{-0.4}^{+0.3}$&$0.933$ &$_{-0.03}^{+0.01}$&$4.0$ &$_{-0.2}^{+0.1}$&$7.09$&$344.0$ &$_{-2.0}^{+0.8}$&$72.7$ &$_{-8.0}^{+4.0}$&$2.41$ &$_{-0.1}^{+0.2}$&$2.3$ &$_{-0.2}^{+0.2}$\\\texttt{M8MA6}&$7.97$ &$_{-0.9}^{+0.4}$&$0.938$ &$_{-0.02}^{+0.02}$&$5.98$ &$_{-0.7}^{+0.3}$&$4.73$&$278.0$ &$_{-1.0}^{+2.0}$&$42.4$ &$_{-1.0}^{+7.0}$&$2.84$ &$_{-0.5}^{+0.2}$&$2.93$ &$_{-0.6}^{+0.3}$\\\texttt{M8MA8}&$7.82$ &$_{-0.4}^{+0.4}$&$0.994$ &$_{-0.02}^{+0.01}$&$7.82$ &$_{-0.4}^{+0.4}$&$3.54$&$247.0$ &$_{-1.0}^{+0.8}$&$31.5$ &$_{-2.0}^{+2.0}$&$3.2$ &$_{-0.3}^{+0.2}$&$3.46$ &$_{-0.3}^{+0.5}$\\\texttt{M8MA10}&$8.06$ &$_{-1.0}^{+0.2}$&$1.01$ &$_{-0.03}^{+0.02}$&$10.1$ &$_{-1.0}^{+0.3}$&$2.84$&$197.0$ &$_{-0.5}^{+1.0}$&$22.3$ &$_{-0.5}^{+1.0}$&$3.72$ &$_{-0.4}^{+0.6}$&$3.89$ &$_{-0.5}^{+0.6}$\\\texttt{M10MA01}&$11.3$ &$_{-1.0}^{+0.3}$&$1.45$ &$_{-0.09}^{+0.07}$&$0.113$ &$_{-0.01}^{+0.003}$&$354.0$&$6.76$ &$_{-1.0}^{+1.0}$&$720.0$ &$_{-200.0}^{+100.0}$&$33.7$ &$_{-7.0}^{+8.0}$&$0.112$ &$_{-0.01}^{+0.003}$\\\texttt{M10MA05}&$10.2$ &$_{-0.3}^{+0.3}$&$1.13$ &$_{-0.02}^{+0.02}$&$0.509$ &$_{-0.02}^{+0.01}$&$70.9$&$143.0$ &$_{-2.0}^{+2.0}$&$420.0$ &$_{-40.0}^{+20.0}$&$4.88$ &$_{-0.5}^{+0.6}$&$0.496$ &$_{-0.02}^{+0.02}$\\\texttt{M10MA1}&$9.72$ &$_{-0.9}^{+0.9}$&$0.868$ &$_{-0.03}^{+0.03}$&$0.972$ &$_{-0.09}^{+0.09}$&$35.4$&$338.0$ &$_{-4.0}^{+3.0}$&$309.0$ &$_{-40.0}^{+20.0}$&$2.79$ &$_{-0.1}^{+0.4}$&$0.888$ &$_{-0.1}^{+0.06}$\\\texttt{M10MA2}&$10.5$ &$_{-0.8}^{+0.3}$&$0.888$ &$_{-0.02}^{+0.02}$&$2.1$ &$_{-0.2}^{+0.07}$&$17.7$&$549.0$ &$_{-1.0}^{+0.9}$&$215.0$ &$_{-10.0}^{+9.0}$&$2.39$ &$_{-0.3}^{+0.1}$&$1.56$ &$_{-0.1}^{+0.2}$\\\texttt{M10MA4}&$10.3$ &$_{-0.4}^{+0.4}$&$0.931$ &$_{-0.03}^{+0.03}$&$4.12$ &$_{-0.2}^{+0.2}$&$8.86$&$529.0$ &$_{-2.0}^{+2.0}$&$112.0$ &$_{-6.0}^{+8.0}$&$2.42$ &$_{-0.2}^{+0.4}$&$2.32$ &$_{-0.2}^{+0.4}$\\\texttt{M10MA6}&$9.78$ &$_{-1.0}^{+0.3}$&$0.952$ &$_{-0.03}^{+0.02}$&$5.87$ &$_{-0.7}^{+0.2}$&$5.91$&$398.0$ &$_{-0.7}^{+2.0}$&$65.2$ &$_{-3.0}^{+7.0}$&$2.7$ &$_{-0.4}^{+0.3}$&$2.77$ &$_{-0.4}^{+0.3}$\\\texttt{M10MA8}&$10.0$ &$_{-0.9}^{+0.4}$&$0.997$ &$_{-0.02}^{+0.02}$&$8.03$ &$_{-0.7}^{+0.3}$&$4.43$&$346.0$ &$_{-1.0}^{+1.0}$&$46.7$ &$_{-1.0}^{+4.0}$&$3.27$ &$_{-0.4}^{+0.4}$&$3.41$ &$_{-0.6}^{+0.4}$\\\texttt{M10MA10}&$9.42$ &$_{-0.5}^{+0.2}$&$0.99$ &$_{-0.01}^{+0.01}$&$9.42$ &$_{-0.5}^{+0.2}$&$3.54$&$288.0$ &$_{-3.0}^{+2.0}$&$34.3$ &$_{-4.0}^{+3.0}$&$3.37$ &$_{-0.2}^{+0.3}$&$3.5$ &$_{-0.3}^{+0.5}$\\\hline
\hline
\end{tabular}\\
\label{tb:simtab}
\end{table*}


==> table_backup.tex <==
\begin{table*}
\caption{Main simulation parameters and derived quantities used throughout this study.}
\centering
\begin{tabular}{l r@{}l r@{}l r@{}l c r@{}l r@{}l r@{}l r@{}l}
\hline
\hline
& \multicolumn{4}{c}{Turbulence} & \multicolumn{3}{c}{Mean $\vecB{B}$-Field} & \multicolumn{6}{c}{Fluctuating $\vecB{B}$-Field} & \multicolumn{2}{c}{Total $\vecB{B}$-Field} \\

\hline

\multicolumn{1}{c}{Simulation ID} & \multicolumn{2}{c}{$\M$} & \multicolumn{2}{c}{$\Exp{\delta v^2}_{\V_{L}}/c_s^2$} & \multicolumn{2}{c}{$\Mao$} & \multicolumn{1}{c}{$B_0/(c_s \sqrt{\rho_0})$} & \multicolumn{2}{c}{$\Exp{\delta B^2}_{\V_L}/(c_s^2 \rho_0)$} & \multicolumn{2}{c}{$\Exp{(\dB\cdot\Bo)^2}^{1/2}_{\V_{L}}/(c_s^2 \rho_0)$} & \multicolumn{2}{c}{$\Maturb$} & \multicolumn{2}{c}{$\Matot$} \\

\multicolumn{1}{c}{(1)} & \multicolumn{2}{c}{(2)} & \multicolumn{2}{c}{(3)} & \multicolumn{2}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{2}{c}{(6)} & \multicolumn{2}{c}{(7)} & \multicolumn{2}{c}{(8)} & \multicolumn{2}{c}{(9)} \\

\hline %simulation                  % Mach                       % kinetic energy                % Ma0                            % B_0          % dB^2                         % dBB0                        % resolution
\texttt{M05Ma100}           & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma10}            & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma1000}          & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma8}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma6}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma4}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma2}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma1}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma05}            & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma01}            & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M05Ma001}           & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma1000}           & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma100}            & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma10}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma8}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma6}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma4}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma2}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma1}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma05}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma01}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M2Ma001}            & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M4Ma100}            & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M4Ma10}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M4Ma8}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M4Ma6}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M4Ma4}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M4Ma2}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M4Ma1}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M4Ma05}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M4Ma01}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M6Ma10}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M6Ma8}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M6Ma6}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M6Ma4}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M6Ma2}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M6Ma1}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M6Ma05}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M6Ma01}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M8Ma10}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M8Ma8}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M8Ma6}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M8Ma4}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M8Ma2}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M8Ma1}              & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M8Ma05}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M8Ma01}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M10Ma10}            & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M10Ma8}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M10Ma6}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M10Ma4}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M10Ma2}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M10Ma1}             & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M10Ma05}            & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\texttt{M10Ma01}            & $x$\,  & $ \pm \Delta x$         & $x$\, & $ \pm \Delta x$         & $x$\,  & $ \pm \Delta x$       & $B_0$        & $x$\, & $\pm \Delta x$        & $x$\, & $\pm \Delta x$     & $x$\, & $\pm \Delta x$  & $x$\, & $\pm \Delta x$\\
\hline 
\hline
\end{tabular} \\
\begin{tablenotes}
\item{\textit{\textbf{Notes:}} Refer to \autoref{app:table_notes} for table notes.}
\end{tablenotes}
\label{tb:simtab}
\end{table*}














 











